What classifiers know what they don't?

Being uncertain when facing the unknown is key to intelligent decision making. However, machine learning algorithms lack reliable estimates about their predictive uncertainty. This leads to wrong and overly-confident decisions when encountering classes unseen during training. Despite the importance of equipping classifiers with uncertainty estimates ready for the real world, prior work has focused on small datasets and little or no class discrepancy between training and testing data. To close this gap, we introduce UIMNET: a realistic, ImageNet-scale test-bed to evaluate predictive uncertainty estimates for deep image classifiers. Our benchmark provides implementations of eight state-of-the-art algorithms, six uncertainty measures, four in-domain metrics, three out-domain metrics, and a fully automated pipeline to train, calibrate, ensemble, select, and evaluate models. Our test-bed is open-source and all of our results are reproducible from a fixed commit in our repository. Adding new datasets, algorithms, measures, or metrics is a matter of a few lines of code-in so hoping that UIMNET becomes a stepping stone towards realistic, rigorous, and reproducible research in uncertainty estimation. Our results show that ensembles of ERM classifiers as well as single MIMO classifiers are the two best alternatives currently available to measure uncertainty about both in-domain and out-domain classes.

==> tables/table_in.tex <==
\begin{table}[h!]
\begin{center}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{llllllll}
\toprule
\textbf{algorithm}& \textbf{spectral}& \textbf{calibration}& \textbf{k}& \textbf{ACC@1}& \textbf{ACC@5}& \textbf{ECE}& \textbf{NLL}\\
\midrule
\multirow{8}{*}{ERM} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.719 \pm 0.002$ &  $0.823 \pm 0.001$ &  $0.051 \pm 0.002$ &  $1.148 \pm 0.004$ \\
            &       &         & 5.0 &  $0.746 \pm 0.001$ &  $0.842 \pm 0.003$ &  $0.044 \pm 0.003$ &  $1.015 \pm 0.009$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.719 \pm 0.002$ &  $0.823 \pm 0.001$ &  $0.032 \pm 0.002$ &  $1.130 \pm 0.004$ \\
            &       &         & 5.0 &  $0.746 \pm 0.001$ &  $0.842 \pm 0.003$ &  $0.022 \pm 0.008$ &  $1.017 \pm 0.016$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.722 \pm 0.001$ &  $0.825 \pm 0.002$ &  $0.049 \pm 0.003$ &  $1.140 \pm 0.009$ \\
            &       &         & 5.0 &  $0.746 \pm 0.002$ &  $0.843 \pm 0.002$ &  $0.047 \pm 0.002$ &  $1.019 \pm 0.005$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.722 \pm 0.001$ &  $0.825 \pm 0.002$ &  $0.031 \pm 0.002$ &  $1.124 \pm 0.008$ \\
            &       &         & 5.0 &  $0.746 \pm 0.002$ &  $0.843 \pm 0.002$ &  $0.017 \pm 0.002$ &  $1.014 \pm 0.005$ \\
\midrule
\multirow{8}{*}{MCDropout} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.721 \pm 0.003$ &  $0.823 \pm 0.002$ &  $0.049 \pm 0.002$ &  $1.133 \pm 0.013$ \\
            &       &         & 5.0 &  $0.745 \pm 0.001$ &  $0.841 \pm 0.001$ &  $0.046 \pm 0.002$ &  $1.019 \pm 0.003$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.721 \pm 0.003$ &  $0.823 \pm 0.002$ &  $0.027 \pm 0.001$ &  $1.118 \pm 0.012$ \\
            &       &         & 5.0 &  $0.745 \pm 0.001$ &  $0.841 \pm 0.001$ &  $0.018 \pm 0.001$ &  $1.014 \pm 0.004$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.722 \pm 0.003$ &  $0.822 \pm 0.002$ &  $0.041 \pm 0.001$ &  $1.139 \pm 0.009$ \\
            &       &         & 5.0 &  $0.745 \pm 0.002$ &  $0.842 \pm 0.001$ &  $0.045 \pm 0.002$ &  $1.019 \pm 0.003$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.722 \pm 0.003$ &  $0.822 \pm 0.002$ &  $0.034 \pm 0.002$ &  $1.129 \pm 0.009$ \\
            &       &         & 5.0 &  $0.745 \pm 0.002$ &  $0.842 \pm 0.001$ &  $0.016 \pm 0.002$ &  $1.015 \pm 0.004$ \\
\midrule
\multirow{8}{*}{MIMO} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.723 \pm 0.001$ &  $0.825 \pm 0.001$ &  $0.044 \pm 0.004$ &  $1.123 \pm 0.001$ \\
            &       &         & 5.0 &  $0.723 \pm 0.003$ &  $0.824 \pm 0.002$ &  $0.089 \pm 0.004$ &  $1.160 \pm 0.003$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.723 \pm 0.001$ &  $0.825 \pm 0.001$ &  $0.028 \pm 0.002$ &  $1.111 \pm 0.001$ \\
            &       &         & 5.0 &  $0.723 \pm 0.003$ &  $0.824 \pm 0.002$ &  $0.015 \pm 0.003$ &  $1.128 \pm 0.006$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.723 \pm 0.001$ &  $0.826 \pm 0.002$ &  $0.045 \pm 0.001$ &  $1.128 \pm 0.004$ \\
            &       &         & 5.0 &  $0.716 \pm 0.011$ &  $0.816 \pm 0.011$ &  $0.090 \pm 0.002$ &  $1.191 \pm 0.047$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.723 \pm 0.001$ &  $0.826 \pm 0.002$ &  $0.030 \pm 0.000$ &  $1.115 \pm 0.005$ \\
            &       &         & 5.0 &  $0.716 \pm 0.011$ &  $0.816 \pm 0.011$ &  $0.014 \pm 0.001$ &  $1.161 \pm 0.048$ \\
\midrule
\multirow{8}{*}{Mixup} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.723 \pm 0.002$ &  $0.825 \pm 0.002$ &  $0.033 \pm 0.003$ &  $1.120 \pm 0.005$ \\
            &       &         & 5.0 &  $0.739 \pm 0.001$ &  $0.837 \pm 0.002$ &  $0.083 \pm 0.000$ &  $1.083 \pm 0.003$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.723 \pm 0.002$ &  $0.825 \pm 0.002$ &  $0.035 \pm 0.001$ &  $1.121 \pm 0.006$ \\
            &       &         & 5.0 &  $0.739 \pm 0.001$ &  $0.837 \pm 0.002$ &  $0.060 \pm 0.056$ &  $1.128 \pm 0.151$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.721 \pm 0.002$ &  $0.824 \pm 0.002$ &  $0.032 \pm 0.002$ &  $1.121 \pm 0.006$ \\
            &       &         & 5.0 &  $0.737 \pm 0.001$ &  $0.837 \pm 0.001$ &  $0.089 \pm 0.004$ &  $1.092 \pm 0.005$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.721 \pm 0.002$ &  $0.824 \pm 0.002$ &  $0.032 \pm 0.001$ &  $1.121 \pm 0.005$ \\
            &       &         & 5.0 &  $0.737 \pm 0.001$ &  $0.837 \pm 0.001$ &  $0.025 \pm 0.004$ &  $1.038 \pm 0.003$ \\
\midrule
\multirow{8}{*}{OC} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.718 \pm 0.005$ &  $0.821 \pm 0.002$ &  $0.045 \pm 0.002$ &  $1.146 \pm 0.005$ \\
            &       &         & 5.0 &  $0.743 \pm 0.001$ &  $0.841 \pm 0.001$ &  $0.045 \pm 0.001$ &  $1.023 \pm 0.001$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.718 \pm 0.001$ &  $0.822 \pm 0.001$ &  $0.031 \pm 0.002$ &  $1.132 \pm 0.002$ \\
            &       &         & 5.0 &  $0.743 \pm 0.001$ &  $0.841 \pm 0.001$ &  $0.016 \pm 0.001$ &  $1.019 \pm 0.002$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.721 \pm 0.003$ &  $0.824 \pm 0.002$ &  $0.049 \pm 0.001$ &  $1.142 \pm 0.009$ \\
            &       &         & 5.0 &  $0.744 \pm 0.002$ &  $0.842 \pm 0.002$ &  $0.046 \pm 0.002$ &  $1.021 \pm 0.003$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.721 \pm 0.003$ &  $0.824 \pm 0.002$ &  $0.032 \pm 0.004$ &  $1.126 \pm 0.009$ \\
            &       &         & 5.0 &  $0.744 \pm 0.002$ &  $0.842 \pm 0.002$ &  $0.015 \pm 0.002$ &  $1.016 \pm 0.002$ \\
\midrule
\multirow{8}{*}{RND} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.719 \pm 0.002$ &  $0.824 \pm 0.000$ &  $0.049 \pm 0.003$ &  $1.136 \pm 0.007$ \\
            &       &         & 5.0 &  $0.743 \pm 0.005$ &  $0.840 \pm 0.003$ &  $0.045 \pm 0.002$ &  $1.029 \pm 0.015$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.719 \pm 0.002$ &  $0.824 \pm 0.000$ &  $0.032 \pm 0.004$ &  $1.121 \pm 0.005$ \\
            &       &         & 5.0 &  $0.743 \pm 0.005$ &  $0.840 \pm 0.003$ &  $0.015 \pm 0.002$ &  $1.023 \pm 0.016$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.718 \pm 0.003$ &  $0.823 \pm 0.002$ &  $0.049 \pm 0.005$ &  $1.139 \pm 0.013$ \\
            &       &         & 5.0 &  $0.745 \pm 0.001$ &  $0.842 \pm 0.001$ &  $0.043 \pm 0.006$ &  $1.018 \pm 0.002$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.718 \pm 0.003$ &  $0.823 \pm 0.002$ &  $0.030 \pm 0.004$ &  $1.124 \pm 0.011$ \\
            &       &         & 5.0 &  $0.745 \pm 0.001$ &  $0.842 \pm 0.001$ &  $0.016 \pm 0.002$ &  $1.015 \pm 0.004$ \\
\midrule
\multirow{8}{*}{SoftLabeler} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.719 \pm 0.001$ &  $0.822 \pm 0.001$ &  $0.036 \pm 0.002$ &  $1.173 \pm 0.006$ \\
            &       &         & 5.0 &  $0.743 \pm 0.003$ &  $0.842 \pm 0.001$ &  $0.136 \pm 0.002$ &  $1.177 \pm 0.012$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.719 \pm 0.001$ &  $0.822 \pm 0.001$ &  $0.054 \pm 0.003$ &  $1.168 \pm 0.007$ \\
            &       &         & 5.0 &  $0.743 \pm 0.003$ &  $0.842 \pm 0.001$ &  $0.044 \pm 0.002$ &  $1.036 \pm 0.009$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.723 \pm 0.004$ &  $0.823 \pm 0.002$ &  $0.038 \pm 0.002$ &  $1.167 \pm 0.010$ \\
            &       &         & 5.0 &  $0.742 \pm 0.001$ &  $0.840 \pm 0.001$ &  $0.136 \pm 0.003$ &  $1.181 \pm 0.006$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.723 \pm 0.004$ &  $0.823 \pm 0.002$ &  $0.051 \pm 0.004$ &  $1.159 \pm 0.010$ \\
            &       &         & 5.0 &  $0.742 \pm 0.001$ &  $0.840 \pm 0.001$ &  $0.044 \pm 0.001$ &  $1.038 \pm 0.001$ \\
\bottomrule
\end{tabular}
}\end{center}
\caption{In-domain results.}\label{table:in-domain-}
\end{table}


==> tables/table_out_Augmentations.tex <==
\begin{table}[h!]
\begin{center}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lllllll}
\toprule
\textbf{algorithm}& \textbf{spectral}& \textbf{calibration}& \textbf{k}& \textbf{AUC}& \textbf{InAsIn}& \textbf{OutAsOut}\\
\midrule
\multirow{8}{*}{ERM} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.656 \pm 0.032$ &  $0.966 \pm 0.030$ &  $0.077 \pm 0.067$ \\
            &       &         & 5.0 &  $0.666 \pm 0.014$ &  $0.966 \pm 0.029$ &  $0.064 \pm 0.055$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.661 \pm 0.035$ &  $0.950 \pm 0.002$ &  $0.104 \pm 0.024$ \\
            &       &         & 5.0 &  $0.665 \pm 0.012$ &  $0.952 \pm 0.002$ &  $0.102 \pm 0.014$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.647 \pm 0.012$ &  $0.951 \pm 0.002$ &  $0.085 \pm 0.016$ \\
            &       &         & 5.0 &  $0.665 \pm 0.007$ &  $0.951 \pm 0.001$ &  $0.103 \pm 0.005$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.647 \pm 0.014$ &  $0.949 \pm 0.003$ &  $0.090 \pm 0.015$ \\
            &       &         & 5.0 &  $0.662 \pm 0.009$ &  $0.951 \pm 0.002$ &  $0.103 \pm 0.004$ \\
\midrule
\multirow{4}{*}{MCDropout} & \multirow{2}{*}{False} & initial & 1.0 &  $0.639 \pm 0.027$ &  $0.965 \pm 0.030$ &  $0.070 \pm 0.061$ \\
            &       & learned & 1.0 &  $0.646 \pm 0.025$ &  $0.950 \pm 0.001$ &  $0.092 \pm 0.022$ \\
            & \multirow{2}{*}{True} & initial & 1.0 &  $0.638 \pm 0.008$ &  $0.951 \pm 0.002$ &  $0.091 \pm 0.016$ \\
            &       & learned & 1.0 &  $0.638 \pm 0.009$ &  $0.950 \pm 0.001$ &  $0.092 \pm 0.014$ \\
\midrule
\multirow{6}{*}{MIMO} & \multirow{2}{*}{False} & initial & 1.0 &  $0.684 \pm 0.015$ &  $0.950 \pm 0.003$ &  $0.123 \pm 0.014$ \\
            &       & learned & 1.0 &  $0.688 \pm 0.014$ &  $0.951 \pm 0.002$ &  $0.120 \pm 0.006$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.671 \pm 0.026$ &  $0.949 \pm 0.001$ &  $0.112 \pm 0.030$ \\
            &       &         & 5.0 &  $0.682 \pm 0.004$ &  $0.950 \pm 0.002$ &  $0.119 \pm 0.004$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.671 \pm 0.032$ &  $0.946 \pm 0.000$ &  $0.117 \pm 0.030$ \\
            &       &         & 5.0 &  $0.676 \pm 0.004$ &  $0.951 \pm 0.002$ &  $0.115 \pm 0.002$ \\
\midrule
\multirow{8}{*}{Mixup} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.678 \pm 0.014$ &  $0.965 \pm 0.030$ &  $0.085 \pm 0.074$ \\
            &       &         & 5.0 &  $0.703 \pm 0.004$ &  $0.966 \pm 0.029$ &  $0.093 \pm 0.081$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.682 \pm 0.016$ &  $0.951 \pm 0.000$ &  $0.122 \pm 0.015$ \\
            &       &         & 5.0 &  $0.693 \pm 0.013$ &  $0.967 \pm 0.029$ &  $0.083 \pm 0.072$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.687 \pm 0.013$ &  $0.951 \pm 0.002$ &  $0.117 \pm 0.014$ \\
            &       &         & 5.0 &  $0.696 \pm 0.003$ &  $0.948 \pm 0.002$ &  $0.130 \pm 0.007$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.684 \pm 0.015$ &  $0.948 \pm 0.002$ &  $0.117 \pm 0.016$ \\
            &       &         & 5.0 &  $0.695 \pm 0.003$ &  $0.949 \pm 0.002$ &  $0.125 \pm 0.007$ \\
\midrule
\multirow{7}{*}{OC} & \multirow{3}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.645 \pm 0.032$ &  $0.949 \pm 0.001$ &  $0.099 \pm 0.015$ \\
            &       &         & 5.0 &  $0.668 \pm 0.011$ &  $0.966 \pm 0.029$ &  $0.070 \pm 0.061$ \\
            &       & learned & 5.0 &  $0.664 \pm 0.012$ &  $0.952 \pm 0.002$ &  $0.099 \pm 0.010$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.670 \pm 0.013$ &  $0.951 \pm 0.001$ &  $0.112 \pm 0.015$ \\
            &       &         & 5.0 &  $0.675 \pm 0.005$ &  $0.965 \pm 0.030$ &  $0.073 \pm 0.063$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.677 \pm 0.015$ &  $0.951 \pm 0.001$ &  $0.112 \pm 0.015$ \\
            &       &         & 5.0 &  $0.672 \pm 0.003$ &  $0.950 \pm 0.003$ &  $0.111 \pm 0.004$ \\
\midrule
\multirow{6}{*}{RND} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.667 \pm 0.023$ &  $0.950 \pm 0.003$ &  $0.118 \pm 0.024$ \\
            &       &         & 5.0 &  $0.668 \pm 0.001$ &  $0.949 \pm 0.004$ &  $0.106 \pm 0.002$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.675 \pm 0.024$ &  $0.949 \pm 0.001$ &  $0.126 \pm 0.024$ \\
            &       &         & 5.0 &  $0.660 \pm 0.003$ &  $0.950 \pm 0.003$ &  $0.109 \pm 0.002$ \\
            & \multirow{2}{*}{True} & initial & 5.0 &  $0.673 \pm 0.003$ &  $0.948 \pm 0.002$ &  $0.110 \pm 0.007$ \\
            &       & learned & 5.0 &  $0.666 \pm 0.003$ &  $0.949 \pm 0.001$ &  $0.106 \pm 0.008$ \\
\midrule
\multirow{8}{*}{SoftLabeler} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.645 \pm 0.019$ &  $0.950 \pm 0.003$ &  $0.097 \pm 0.011$ \\
            &       &         & 5.0 &  $0.651 \pm 0.010$ &  $0.983 \pm 0.030$ &  $0.028 \pm 0.048$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.646 \pm 0.020$ &  $0.950 \pm 0.004$ &  $0.098 \pm 0.015$ \\
            &       &         & 5.0 &  $0.656 \pm 0.007$ &  $0.966 \pm 0.029$ &  $0.066 \pm 0.057$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.650 \pm 0.024$ &  $0.951 \pm 0.001$ &  $0.099 \pm 0.022$ \\
            &       &         & 5.0 &  $0.654 \pm 0.008$ &  $0.951 \pm 0.001$ &  $0.099 \pm 0.007$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.648 \pm 0.021$ &  $0.950 \pm 0.001$ &  $0.099 \pm 0.020$ \\
            &       &         & 5.0 &  $0.655 \pm 0.008$ &  $0.950 \pm 0.004$ &  $0.097 \pm 0.007$ \\
\bottomrule
\end{tabular}
}\end{center}
\caption{Out-domain results for measure Augmentations}\label{table:out-domain-Augmentations}
\end{table}


==> tables/table_out_Entropy.tex <==
\begin{table}[h!]
\begin{center}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lllllll}
\toprule
\textbf{algorithm}& \textbf{spectral}& \textbf{calibration}& \textbf{k}& \textbf{AUC}& \textbf{InAsIn}& \textbf{OutAsOut}\\
\midrule
\multirow{8}{*}{ERM} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.804 \pm 0.011$ &  $0.938 \pm 0.001$ &  $0.255 \pm 0.015$ \\
            &       &         & 5.0 &  $0.834 \pm 0.004$ &  $0.938 \pm 0.003$ &  $0.277 \pm 0.010$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.805 \pm 0.011$ &  $0.938 \pm 0.002$ &  $0.255 \pm 0.017$ \\
            &       &         & 5.0 &  $0.829 \pm 0.004$ &  $0.938 \pm 0.004$ &  $0.280 \pm 0.010$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.819 \pm 0.010$ &  $0.940 \pm 0.001$ &  $0.259 \pm 0.021$ \\
            &       &         & 5.0 &  $0.830 \pm 0.007$ &  $0.938 \pm 0.002$ &  $0.268 \pm 0.015$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.821 \pm 0.011$ &  $0.941 \pm 0.000$ &  $0.257 \pm 0.019$ \\
            &       &         & 5.0 &  $0.827 \pm 0.006$ &  $0.937 \pm 0.001$ &  $0.272 \pm 0.012$ \\
\midrule
\multirow{8}{*}{MCDropout} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.811 \pm 0.002$ &  $0.940 \pm 0.004$ &  $0.256 \pm 0.012$ \\
            &       &         & 5.0 &  $0.831 \pm 0.003$ &  $0.940 \pm 0.002$ &  $0.268 \pm 0.011$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.812 \pm 0.003$ &  $0.941 \pm 0.004$ &  $0.255 \pm 0.016$ \\
            &       &         & 5.0 &  $0.829 \pm 0.002$ &  $0.940 \pm 0.002$ &  $0.271 \pm 0.009$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.812 \pm 0.007$ &  $0.940 \pm 0.001$ &  $0.252 \pm 0.006$ \\
            &       &         & 5.0 &  $0.832 \pm 0.006$ &  $0.939 \pm 0.002$ &  $0.266 \pm 0.013$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.814 \pm 0.007$ &  $0.940 \pm 0.001$ &  $0.252 \pm 0.005$ \\
            &       &         & 5.0 &  $0.829 \pm 0.004$ &  $0.939 \pm 0.002$ &  $0.267 \pm 0.010$ \\
\midrule
\multirow{8}{*}{MIMO} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.810 \pm 0.002$ &  $0.940 \pm 0.000$ &  $0.257 \pm 0.005$ \\
            &       &         & 5.0 &  $0.821 \pm 0.007$ &  $0.937 \pm 0.001$ &  $0.249 \pm 0.007$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.811 \pm 0.002$ &  $0.940 \pm 0.001$ &  $0.258 \pm 0.006$ \\
            &       &         & 5.0 &  $0.818 \pm 0.006$ &  $0.937 \pm 0.000$ &  $0.251 \pm 0.009$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.815 \pm 0.002$ &  $0.941 \pm 0.003$ &  $0.257 \pm 0.014$ \\
            &       &         & 5.0 &  $0.818 \pm 0.003$ &  $0.940 \pm 0.001$ &  $0.236 \pm 0.004$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.817 \pm 0.001$ &  $0.941 \pm 0.003$ &  $0.257 \pm 0.012$ \\
            &       &         & 5.0 &  $0.813 \pm 0.004$ &  $0.939 \pm 0.001$ &  $0.240 \pm 0.005$ \\
\midrule
\multirow{8}{*}{Mixup} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.815 \pm 0.002$ &  $0.940 \pm 0.002$ &  $0.256 \pm 0.006$ \\
            &       &         & 5.0 &  $0.824 \pm 0.002$ &  $0.938 \pm 0.002$ &  $0.257 \pm 0.013$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.815 \pm 0.002$ &  $0.940 \pm 0.002$ &  $0.256 \pm 0.007$ \\
            &       &         & 5.0 &  $0.814 \pm 0.013$ &  $0.938 \pm 0.000$ &  $0.260 \pm 0.013$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.805 \pm 0.006$ &  $0.939 \pm 0.002$ &  $0.242 \pm 0.021$ \\
            &       &         & 5.0 &  $0.820 \pm 0.003$ &  $0.938 \pm 0.002$ &  $0.256 \pm 0.008$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.805 \pm 0.006$ &  $0.939 \pm 0.002$ &  $0.243 \pm 0.020$ \\
            &       &         & 5.0 &  $0.819 \pm 0.001$ &  $0.938 \pm 0.001$ &  $0.258 \pm 0.008$ \\
\midrule
\multirow{8}{*}{OC} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.814 \pm 0.009$ &  $0.940 \pm 0.001$ &  $0.258 \pm 0.015$ \\
            &       &         & 5.0 &  $0.829 \pm 0.008$ &  $0.939 \pm 0.003$ &  $0.269 \pm 0.017$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.807 \pm 0.015$ &  $0.939 \pm 0.004$ &  $0.253 \pm 0.028$ \\
            &       &         & 5.0 &  $0.826 \pm 0.008$ &  $0.938 \pm 0.002$ &  $0.272 \pm 0.014$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.810 \pm 0.006$ &  $0.939 \pm 0.002$ &  $0.255 \pm 0.021$ \\
            &       &         & 5.0 &  $0.831 \pm 0.004$ &  $0.938 \pm 0.002$ &  $0.268 \pm 0.014$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.813 \pm 0.007$ &  $0.939 \pm 0.002$ &  $0.254 \pm 0.023$ \\
            &       &         & 5.0 &  $0.828 \pm 0.003$ &  $0.937 \pm 0.002$ &  $0.272 \pm 0.015$ \\
\midrule
\multirow{8}{*}{RND} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.818 \pm 0.006$ &  $0.939 \pm 0.001$ &  $0.272 \pm 0.015$ \\
            &       &         & 5.0 &  $0.831 \pm 0.004$ &  $0.940 \pm 0.003$ &  $0.267 \pm 0.014$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.821 \pm 0.006$ &  $0.939 \pm 0.000$ &  $0.268 \pm 0.012$ \\
            &       &         & 5.0 &  $0.829 \pm 0.004$ &  $0.939 \pm 0.003$ &  $0.269 \pm 0.013$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.818 \pm 0.015$ &  $0.940 \pm 0.002$ &  $0.268 \pm 0.024$ \\
            &       &         & 5.0 &  $0.830 \pm 0.008$ &  $0.938 \pm 0.002$ &  $0.268 \pm 0.016$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.820 \pm 0.016$ &  $0.940 \pm 0.001$ &  $0.267 \pm 0.024$ \\
            &       &         & 5.0 &  $0.827 \pm 0.008$ &  $0.937 \pm 0.001$ &  $0.270 \pm 0.016$ \\
\midrule
\multirow{8}{*}{SoftLabeler} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.785 \pm 0.010$ &  $0.940 \pm 0.000$ &  $0.218 \pm 0.014$ \\
            &       &         & 5.0 &  $0.809 \pm 0.002$ &  $0.940 \pm 0.001$ &  $0.237 \pm 0.005$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.789 \pm 0.008$ &  $0.940 \pm 0.000$ &  $0.226 \pm 0.012$ \\
            &       &         & 5.0 &  $0.813 \pm 0.003$ &  $0.940 \pm 0.001$ &  $0.247 \pm 0.004$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.789 \pm 0.004$ &  $0.941 \pm 0.002$ &  $0.214 \pm 0.010$ \\
            &       &         & 5.0 &  $0.801 \pm 0.009$ &  $0.939 \pm 0.001$ &  $0.230 \pm 0.007$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.792 \pm 0.004$ &  $0.940 \pm 0.002$ &  $0.222 \pm 0.005$ \\
            &       &         & 5.0 &  $0.807 \pm 0.007$ &  $0.939 \pm 0.001$ &  $0.242 \pm 0.004$ \\
\bottomrule
\end{tabular}
}\end{center}
\caption{Out-domain results for measure Entropy}\label{table:out-domain-Entropy}
\end{table}


==> tables/table_out_Gap.tex <==
\begin{table}[h!]
\begin{center}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lllllll}
\toprule
\textbf{algorithm}& \textbf{spectral}& \textbf{calibration}& \textbf{k}& \textbf{AUC}& \textbf{InAsIn}& \textbf{OutAsOut}\\
\midrule
\multirow{8}{*}{ERM} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.774 \pm 0.009$ &  $0.942 \pm 0.002$ &  $0.175 \pm 0.008$ \\
            &       &         & 5.0 &  $0.797 \pm 0.002$ &  $0.942 \pm 0.005$ &  $0.190 \pm 0.011$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.777 \pm 0.009$ &  $0.941 \pm 0.001$ &  $0.178 \pm 0.009$ \\
            &       &         & 5.0 &  $0.791 \pm 0.002$ &  $0.943 \pm 0.004$ &  $0.181 \pm 0.009$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.784 \pm 0.007$ &  $0.944 \pm 0.002$ &  $0.180 \pm 0.013$ \\
            &       &         & 5.0 &  $0.796 \pm 0.004$ &  $0.943 \pm 0.000$ &  $0.185 \pm 0.009$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.788 \pm 0.009$ &  $0.944 \pm 0.003$ &  $0.185 \pm 0.016$ \\
            &       &         & 5.0 &  $0.791 \pm 0.004$ &  $0.943 \pm 0.001$ &  $0.178 \pm 0.008$ \\
\midrule
\multirow{8}{*}{MCDropout} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.780 \pm 0.002$ &  $0.945 \pm 0.001$ &  $0.176 \pm 0.003$ \\
            &       &         & 5.0 &  $0.796 \pm 0.002$ &  $0.941 \pm 0.001$ &  $0.186 \pm 0.011$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.783 \pm 0.002$ &  $0.945 \pm 0.001$ &  $0.179 \pm 0.003$ \\
            &       &         & 5.0 &  $0.791 \pm 0.002$ &  $0.941 \pm 0.001$ &  $0.178 \pm 0.009$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.779 \pm 0.002$ &  $0.945 \pm 0.002$ &  $0.171 \pm 0.001$ \\
            &       &         & 5.0 &  $0.796 \pm 0.001$ &  $0.942 \pm 0.000$ &  $0.185 \pm 0.004$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.781 \pm 0.002$ &  $0.945 \pm 0.002$ &  $0.173 \pm 0.001$ \\
            &       &         & 5.0 &  $0.791 \pm 0.001$ &  $0.943 \pm 0.001$ &  $0.179 \pm 0.004$ \\
\midrule
\multirow{8}{*}{MIMO} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.778 \pm 0.002$ &  $0.942 \pm 0.000$ &  $0.175 \pm 0.005$ \\
            &       &         & 5.0 &  $0.788 \pm 0.001$ &  $0.944 \pm 0.001$ &  $0.176 \pm 0.005$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.781 \pm 0.002$ &  $0.942 \pm 0.000$ &  $0.179 \pm 0.004$ \\
            &       &         & 5.0 &  $0.779 \pm 0.001$ &  $0.944 \pm 0.001$ &  $0.166 \pm 0.005$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.781 \pm 0.003$ &  $0.944 \pm 0.003$ &  $0.176 \pm 0.003$ \\
            &       &         & 5.0 &  $0.783 \pm 0.006$ &  $0.943 \pm 0.001$ &  $0.174 \pm 0.006$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.784 \pm 0.003$ &  $0.944 \pm 0.003$ &  $0.180 \pm 0.005$ \\
            &       &         & 5.0 &  $0.774 \pm 0.007$ &  $0.943 \pm 0.002$ &  $0.167 \pm 0.005$ \\
\midrule
\multirow{8}{*}{Mixup} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.782 \pm 0.004$ &  $0.944 \pm 0.002$ &  $0.177 \pm 0.004$ \\
            &       &         & 5.0 &  $0.794 \pm 0.002$ &  $0.942 \pm 0.002$ &  $0.183 \pm 0.009$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.781 \pm 0.004$ &  $0.944 \pm 0.002$ &  $0.176 \pm 0.004$ \\
            &       &         & 5.0 &  $0.781 \pm 0.009$ &  $0.944 \pm 0.002$ &  $0.165 \pm 0.017$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.780 \pm 0.002$ &  $0.945 \pm 0.003$ &  $0.172 \pm 0.011$ \\
            &       &         & 5.0 &  $0.795 \pm 0.003$ &  $0.942 \pm 0.001$ &  $0.189 \pm 0.002$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.780 \pm 0.002$ &  $0.945 \pm 0.002$ &  $0.172 \pm 0.011$ \\
            &       &         & 5.0 &  $0.786 \pm 0.003$ &  $0.943 \pm 0.001$ &  $0.177 \pm 0.002$ \\
\midrule
\multirow{8}{*}{OC} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.779 \pm 0.007$ &  $0.942 \pm 0.002$ &  $0.181 \pm 0.015$ \\
            &       &         & 5.0 &  $0.794 \pm 0.005$ &  $0.943 \pm 0.001$ &  $0.186 \pm 0.012$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.777 \pm 0.009$ &  $0.943 \pm 0.003$ &  $0.180 \pm 0.010$ \\
            &       &         & 5.0 &  $0.789 \pm 0.005$ &  $0.944 \pm 0.001$ &  $0.178 \pm 0.011$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.780 \pm 0.004$ &  $0.944 \pm 0.001$ &  $0.175 \pm 0.004$ \\
            &       &         & 5.0 &  $0.798 \pm 0.004$ &  $0.941 \pm 0.002$ &  $0.186 \pm 0.007$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.784 \pm 0.006$ &  $0.944 \pm 0.000$ &  $0.181 \pm 0.008$ \\
            &       &         & 5.0 &  $0.793 \pm 0.004$ &  $0.941 \pm 0.003$ &  $0.181 \pm 0.008$ \\
\midrule
\multirow{8}{*}{RND} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.783 \pm 0.001$ &  $0.943 \pm 0.003$ &  $0.185 \pm 0.003$ \\
            &       &         & 5.0 &  $0.796 \pm 0.005$ &  $0.943 \pm 0.001$ &  $0.183 \pm 0.013$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.787 \pm 0.000$ &  $0.943 \pm 0.003$ &  $0.191 \pm 0.003$ \\
            &       &         & 5.0 &  $0.791 \pm 0.005$ &  $0.943 \pm 0.001$ &  $0.176 \pm 0.010$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.781 \pm 0.010$ &  $0.943 \pm 0.001$ &  $0.180 \pm 0.008$ \\
            &       &         & 5.0 &  $0.794 \pm 0.006$ &  $0.941 \pm 0.001$ &  $0.188 \pm 0.003$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.784 \pm 0.011$ &  $0.943 \pm 0.001$ &  $0.184 \pm 0.010$ \\
            &       &         & 5.0 &  $0.790 \pm 0.007$ &  $0.941 \pm 0.002$ &  $0.182 \pm 0.003$ \\
\midrule
\multirow{8}{*}{SoftLabeler} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.771 \pm 0.006$ &  $0.942 \pm 0.002$ &  $0.175 \pm 0.007$ \\
            &       &         & 5.0 &  $0.791 \pm 0.005$ &  $0.943 \pm 0.002$ &  $0.179 \pm 0.002$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.769 \pm 0.005$ &  $0.943 \pm 0.003$ &  $0.170 \pm 0.007$ \\
            &       &         & 5.0 &  $0.782 \pm 0.005$ &  $0.944 \pm 0.002$ &  $0.169 \pm 0.001$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.771 \pm 0.004$ &  $0.944 \pm 0.002$ &  $0.171 \pm 0.005$ \\
            &       &         & 5.0 &  $0.787 \pm 0.006$ &  $0.940 \pm 0.002$ &  $0.183 \pm 0.003$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.767 \pm 0.004$ &  $0.944 \pm 0.002$ &  $0.164 \pm 0.003$ \\
            &       &         & 5.0 &  $0.779 \pm 0.005$ &  $0.941 \pm 0.003$ &  $0.172 \pm 0.003$ \\
\bottomrule
\end{tabular}
}\end{center}
\caption{Out-domain results for measure Gap}\label{table:out-domain-Gap}
\end{table}


==> tables/table_out_Jacobian.tex <==
\begin{table}[h!]
\begin{center}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lllllll}
\toprule
\textbf{algorithm}& \textbf{spectral}& \textbf{calibration}& \textbf{k}& \textbf{AUC}& \textbf{InAsIn}& \textbf{OutAsOut}\\
\midrule
\multirow{8}{*}{ERM} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.553 \pm 0.011$ &  $0.958 \pm 0.002$ &  $0.046 \pm 0.009$ \\
            &       &         & 5.0 &  $0.211 \pm 0.005$ &  $0.960 \pm 0.001$ &  $0.001 \pm 0.000$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.553 \pm 0.011$ &  $0.958 \pm 0.002$ &  $0.046 \pm 0.009$ \\
            &       &         & 5.0 &  $0.211 \pm 0.005$ &  $0.960 \pm 0.001$ &  $0.001 \pm 0.000$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.541 \pm 0.028$ &  $0.958 \pm 0.002$ &  $0.042 \pm 0.013$ \\
            &       &         & 5.0 &  $0.218 \pm 0.011$ &  $0.960 \pm 0.002$ &  $0.001 \pm 0.000$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.541 \pm 0.028$ &  $0.958 \pm 0.002$ &  $0.042 \pm 0.013$ \\
            &       &         & 5.0 &  $0.218 \pm 0.011$ &  $0.960 \pm 0.002$ &  $0.001 \pm 0.000$ \\
\midrule
\multirow{8}{*}{MIMO} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.278 \pm 0.008$ &  $0.962 \pm 0.002$ &  $0.003 \pm 0.001$ \\
            &       &         & 5.0 &  $0.239 \pm 0.010$ &  $0.959 \pm 0.001$ &  $0.001 \pm 0.000$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.278 \pm 0.008$ &  $0.962 \pm 0.002$ &  $0.003 \pm 0.001$ \\
            &       &         & 5.0 &  $0.239 \pm 0.010$ &  $0.959 \pm 0.001$ &  $0.001 \pm 0.000$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.269 \pm 0.002$ &  $0.961 \pm 0.001$ &  $0.003 \pm 0.000$ \\
            &       &         & 5.0 &  $0.241 \pm 0.011$ &  $0.959 \pm 0.001$ &  $0.001 \pm 0.000$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.269 \pm 0.002$ &  $0.961 \pm 0.001$ &  $0.003 \pm 0.000$ \\
            &       &         & 5.0 &  $0.241 \pm 0.011$ &  $0.959 \pm 0.001$ &  $0.001 \pm 0.000$ \\
\midrule
\multirow{8}{*}{Mixup} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.569 \pm 0.007$ &  $0.953 \pm 0.002$ &  $0.054 \pm 0.003$ \\
            &       &         & 5.0 &  $0.251 \pm 0.002$ &  $0.960 \pm 0.001$ &  $0.001 \pm 0.000$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.569 \pm 0.007$ &  $0.953 \pm 0.002$ &  $0.054 \pm 0.003$ \\
            &       &         & 5.0 &  $0.251 \pm 0.002$ &  $0.960 \pm 0.001$ &  $0.001 \pm 0.000$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.547 \pm 0.022$ &  $0.955 \pm 0.002$ &  $0.047 \pm 0.009$ \\
            &       &         & 5.0 &  $0.259 \pm 0.003$ &  $0.960 \pm 0.003$ &  $0.001 \pm 0.000$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.547 \pm 0.022$ &  $0.955 \pm 0.002$ &  $0.047 \pm 0.009$ \\
            &       &         & 5.0 &  $0.259 \pm 0.003$ &  $0.960 \pm 0.003$ &  $0.001 \pm 0.000$ \\
\midrule
\multirow{8}{*}{OC} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.554 \pm 0.009$ &  $0.956 \pm 0.001$ &  $0.049 \pm 0.006$ \\
            &       &         & 5.0 &  $0.223 \pm 0.011$ &  $0.961 \pm 0.002$ &  $0.001 \pm 0.000$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.532 \pm 0.016$ &  $0.958 \pm 0.001$ &  $0.038 \pm 0.003$ \\
            &       &         & 5.0 &  $0.223 \pm 0.011$ &  $0.961 \pm 0.002$ &  $0.001 \pm 0.000$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.549 \pm 0.022$ &  $0.958 \pm 0.002$ &  $0.046 \pm 0.011$ \\
            &       &         & 5.0 &  $0.219 \pm 0.002$ &  $0.961 \pm 0.001$ &  $0.000 \pm 0.000$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.549 \pm 0.022$ &  $0.958 \pm 0.002$ &  $0.046 \pm 0.011$ \\
            &       &         & 5.0 &  $0.219 \pm 0.002$ &  $0.961 \pm 0.001$ &  $0.000 \pm 0.000$ \\
\midrule
\multirow{8}{*}{RND} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.545 \pm 0.001$ &  $0.955 \pm 0.003$ &  $0.046 \pm 0.000$ \\
            &       &         & 5.0 &  $0.218 \pm 0.003$ &  $0.960 \pm 0.003$ &  $0.000 \pm 0.000$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.545 \pm 0.001$ &  $0.955 \pm 0.003$ &  $0.046 \pm 0.000$ \\
            &       &         & 5.0 &  $0.218 \pm 0.003$ &  $0.960 \pm 0.003$ &  $0.000 \pm 0.000$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.520 \pm 0.029$ &  $0.956 \pm 0.000$ &  $0.038 \pm 0.005$ \\
            &       &         & 5.0 &  $0.220 \pm 0.011$ &  $0.960 \pm 0.002$ &  $0.001 \pm 0.000$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.520 \pm 0.029$ &  $0.956 \pm 0.000$ &  $0.038 \pm 0.005$ \\
            &       &         & 5.0 &  $0.220 \pm 0.011$ &  $0.960 \pm 0.002$ &  $0.001 \pm 0.000$ \\
\midrule
\multirow{8}{*}{SoftLabeler} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.587 \pm 0.009$ &  $0.954 \pm 0.001$ &  $0.047 \pm 0.002$ \\
            &       &         & 5.0 &  $0.394 \pm 0.011$ &  $0.956 \pm 0.001$ &  $0.019 \pm 0.003$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.587 \pm 0.009$ &  $0.954 \pm 0.001$ &  $0.047 \pm 0.002$ \\
            &       &         & 5.0 &  $0.394 \pm 0.011$ &  $0.956 \pm 0.001$ &  $0.019 \pm 0.003$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.585 \pm 0.009$ &  $0.952 \pm 0.003$ &  $0.046 \pm 0.006$ \\
            &       &         & 5.0 &  $0.400 \pm 0.018$ &  $0.956 \pm 0.001$ &  $0.018 \pm 0.002$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.585 \pm 0.009$ &  $0.952 \pm 0.003$ &  $0.046 \pm 0.006$ \\
            &       &         & 5.0 &  $0.400 \pm 0.018$ &  $0.956 \pm 0.001$ &  $0.018 \pm 0.002$ \\
\bottomrule
\end{tabular}
}\end{center}
\caption{Out-domain results for measure Jacobian}\label{table:out-domain-Jacobian}
\end{table}


==> tables/table_out_Largest.tex <==
\begin{table}[h!]
\begin{center}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lllllll}
\toprule
\textbf{algorithm}& \textbf{spectral}& \textbf{calibration}& \textbf{k}& \textbf{AUC}& \textbf{InAsIn}& \textbf{OutAsOut}\\
\midrule
\multirow{8}{*}{ERM} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.792 \pm 0.010$ &  $0.939 \pm 0.002$ &  $0.239 \pm 0.016$ \\
            &       &         & 5.0 &  $0.821 \pm 0.002$ &  $0.940 \pm 0.003$ &  $0.269 \pm 0.007$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.796 \pm 0.010$ &  $0.939 \pm 0.002$ &  $0.243 \pm 0.015$ \\
            &       &         & 5.0 &  $0.812 \pm 0.004$ &  $0.940 \pm 0.003$ &  $0.260 \pm 0.008$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.804 \pm 0.009$ &  $0.941 \pm 0.001$ &  $0.249 \pm 0.021$ \\
            &       &         & 5.0 &  $0.819 \pm 0.005$ &  $0.938 \pm 0.001$ &  $0.265 \pm 0.011$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.810 \pm 0.010$ &  $0.941 \pm 0.001$ &  $0.251 \pm 0.021$ \\
            &       &         & 5.0 &  $0.812 \pm 0.005$ &  $0.939 \pm 0.000$ &  $0.256 \pm 0.008$ \\
\midrule
\multirow{8}{*}{MCDropout} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.798 \pm 0.002$ &  $0.942 \pm 0.002$ &  $0.241 \pm 0.004$ \\
            &       &         & 5.0 &  $0.820 \pm 0.001$ &  $0.941 \pm 0.003$ &  $0.260 \pm 0.007$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.802 \pm 0.001$ &  $0.942 \pm 0.002$ &  $0.245 \pm 0.006$ \\
            &       &         & 5.0 &  $0.813 \pm 0.001$ &  $0.940 \pm 0.004$ &  $0.250 \pm 0.007$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.798 \pm 0.004$ &  $0.941 \pm 0.002$ &  $0.242 \pm 0.006$ \\
            &       &         & 5.0 &  $0.820 \pm 0.003$ &  $0.939 \pm 0.002$ &  $0.261 \pm 0.009$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.801 \pm 0.004$ &  $0.941 \pm 0.002$ &  $0.242 \pm 0.006$ \\
            &       &         & 5.0 &  $0.813 \pm 0.002$ &  $0.940 \pm 0.002$ &  $0.254 \pm 0.010$ \\
\midrule
\multirow{8}{*}{MIMO} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.797 \pm 0.002$ &  $0.940 \pm 0.002$ &  $0.244 \pm 0.005$ \\
            &       &         & 5.0 &  $0.813 \pm 0.005$ &  $0.938 \pm 0.000$ &  $0.249 \pm 0.006$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.801 \pm 0.002$ &  $0.940 \pm 0.001$ &  $0.249 \pm 0.004$ \\
            &       &         & 5.0 &  $0.801 \pm 0.004$ &  $0.939 \pm 0.000$ &  $0.242 \pm 0.004$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.801 \pm 0.003$ &  $0.941 \pm 0.000$ &  $0.245 \pm 0.004$ \\
            &       &         & 5.0 &  $0.809 \pm 0.004$ &  $0.939 \pm 0.002$ &  $0.238 \pm 0.001$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.805 \pm 0.003$ &  $0.942 \pm 0.000$ &  $0.247 \pm 0.005$ \\
            &       &         & 5.0 &  $0.797 \pm 0.005$ &  $0.938 \pm 0.001$ &  $0.234 \pm 0.002$ \\
\midrule
\multirow{8}{*}{Mixup} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.802 \pm 0.003$ &  $0.940 \pm 0.001$ &  $0.247 \pm 0.009$ \\
            &       &         & 5.0 &  $0.818 \pm 0.001$ &  $0.939 \pm 0.001$ &  $0.257 \pm 0.006$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.802 \pm 0.003$ &  $0.940 \pm 0.001$ &  $0.245 \pm 0.009$ \\
            &       &         & 5.0 &  $0.798 \pm 0.014$ &  $0.939 \pm 0.001$ &  $0.235 \pm 0.023$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.797 \pm 0.003$ &  $0.940 \pm 0.002$ &  $0.237 \pm 0.016$ \\
            &       &         & 5.0 &  $0.816 \pm 0.002$ &  $0.938 \pm 0.002$ &  $0.259 \pm 0.010$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.797 \pm 0.003$ &  $0.940 \pm 0.002$ &  $0.237 \pm 0.015$ \\
            &       &         & 5.0 &  $0.805 \pm 0.002$ &  $0.940 \pm 0.001$ &  $0.249 \pm 0.008$ \\
\midrule
\multirow{8}{*}{OC} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.799 \pm 0.008$ &  $0.940 \pm 0.001$ &  $0.249 \pm 0.016$ \\
            &       &         & 5.0 &  $0.818 \pm 0.007$ &  $0.939 \pm 0.001$ &  $0.266 \pm 0.013$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.796 \pm 0.012$ &  $0.941 \pm 0.004$ &  $0.245 \pm 0.022$ \\
            &       &         & 5.0 &  $0.811 \pm 0.007$ &  $0.939 \pm 0.001$ &  $0.257 \pm 0.013$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.798 \pm 0.005$ &  $0.941 \pm 0.002$ &  $0.244 \pm 0.015$ \\
            &       &         & 5.0 &  $0.820 \pm 0.003$ &  $0.938 \pm 0.001$ &  $0.261 \pm 0.008$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.803 \pm 0.007$ &  $0.940 \pm 0.002$ &  $0.248 \pm 0.016$ \\
            &       &         & 5.0 &  $0.814 \pm 0.003$ &  $0.938 \pm 0.001$ &  $0.252 \pm 0.010$ \\
\midrule
\multirow{8}{*}{RND} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.803 \pm 0.004$ &  $0.939 \pm 0.001$ &  $0.261 \pm 0.008$ \\
            &       &         & 5.0 &  $0.820 \pm 0.004$ &  $0.938 \pm 0.002$ &  $0.264 \pm 0.012$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.809 \pm 0.004$ &  $0.939 \pm 0.000$ &  $0.266 \pm 0.008$ \\
            &       &         & 5.0 &  $0.813 \pm 0.004$ &  $0.939 \pm 0.000$ &  $0.256 \pm 0.011$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.802 \pm 0.013$ &  $0.939 \pm 0.002$ &  $0.254 \pm 0.018$ \\
            &       &         & 5.0 &  $0.818 \pm 0.006$ &  $0.938 \pm 0.001$ &  $0.261 \pm 0.009$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.806 \pm 0.014$ &  $0.939 \pm 0.002$ &  $0.257 \pm 0.018$ \\
            &       &         & 5.0 &  $0.811 \pm 0.008$ &  $0.938 \pm 0.001$ &  $0.256 \pm 0.008$ \\
\midrule
\multirow{8}{*}{SoftLabeler} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.785 \pm 0.007$ &  $0.940 \pm 0.001$ &  $0.224 \pm 0.011$ \\
            &       &         & 5.0 &  $0.810 \pm 0.004$ &  $0.940 \pm 0.001$ &  $0.246 \pm 0.004$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.782 \pm 0.007$ &  $0.941 \pm 0.001$ &  $0.222 \pm 0.011$ \\
            &       &         & 5.0 &  $0.800 \pm 0.004$ &  $0.941 \pm 0.000$ &  $0.238 \pm 0.002$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.788 \pm 0.005$ &  $0.940 \pm 0.001$ &  $0.222 \pm 0.006$ \\
            &       &         & 5.0 &  $0.805 \pm 0.007$ &  $0.939 \pm 0.001$ &  $0.239 \pm 0.005$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.783 \pm 0.005$ &  $0.940 \pm 0.001$ &  $0.222 \pm 0.005$ \\
            &       &         & 5.0 &  $0.796 \pm 0.006$ &  $0.940 \pm 0.001$ &  $0.236 \pm 0.005$ \\
\bottomrule
\end{tabular}
}\end{center}
\caption{Out-domain results for measure Largest}\label{table:out-domain-Largest}
\end{table}


==> tables/table_out_Native.tex <==
\begin{table}[h!]
\begin{center}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lllllll}
\toprule
\textbf{algorithm}& \textbf{spectral}& \textbf{calibration}& \textbf{k}& \textbf{AUC}& \textbf{InAsIn}& \textbf{OutAsOut}\\
\midrule
\multirow{4}{*}{ERM} & \multirow{2}{*}{False} & initial & 5.0 &  $0.773 \pm 0.004$ &  $0.941 \pm 0.003$ &  $0.133 \pm 0.003$ \\
            &       & learned & 5.0 &  $0.773 \pm 0.004$ &  $0.941 \pm 0.003$ &  $0.133 \pm 0.003$ \\
            & \multirow{2}{*}{True} & initial & 5.0 &  $0.769 \pm 0.001$ &  $0.942 \pm 0.001$ &  $0.121 \pm 0.004$ \\
            &       & learned & 5.0 &  $0.769 \pm 0.001$ &  $0.942 \pm 0.001$ &  $0.121 \pm 0.004$ \\
\midrule
\multirow{8}{*}{MCDropout} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.519 \pm 0.004$ &  $0.960 \pm 0.001$ &  $0.095 \pm 0.004$ \\
            &       &         & 5.0 &  $0.770 \pm 0.003$ &  $0.942 \pm 0.001$ &  $0.128 \pm 0.007$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.519 \pm 0.004$ &  $0.960 \pm 0.001$ &  $0.095 \pm 0.004$ \\
            &       &         & 5.0 &  $0.770 \pm 0.003$ &  $0.942 \pm 0.001$ &  $0.128 \pm 0.007$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.519 \pm 0.004$ &  $0.959 \pm 0.001$ &  $0.099 \pm 0.004$ \\
            &       &         & 5.0 &  $0.770 \pm 0.002$ &  $0.941 \pm 0.002$ &  $0.123 \pm 0.006$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.519 \pm 0.004$ &  $0.959 \pm 0.001$ &  $0.099 \pm 0.004$ \\
            &       &         & 5.0 &  $0.770 \pm 0.002$ &  $0.941 \pm 0.002$ &  $0.123 \pm 0.006$ \\
\midrule
\multirow{4}{*}{MIMO} & \multirow{2}{*}{False} & initial & 5.0 &  $0.734 \pm 0.007$ &  $0.947 \pm 0.002$ &  $0.089 \pm 0.011$ \\
            &       & learned & 5.0 &  $0.734 \pm 0.007$ &  $0.947 \pm 0.002$ &  $0.089 \pm 0.011$ \\
            & \multirow{2}{*}{True} & initial & 5.0 &  $0.721 \pm 0.013$ &  $0.945 \pm 0.004$ &  $0.080 \pm 0.015$ \\
            &       & learned & 5.0 &  $0.721 \pm 0.013$ &  $0.945 \pm 0.004$ &  $0.080 \pm 0.015$ \\
\midrule
\multirow{8}{*}{Mixup} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.439 \pm 0.009$ &  $0.944 \pm 0.002$ &  $0.040 \pm 0.002$ \\
            &       &         & 5.0 &  $0.752 \pm 0.005$ &  $0.943 \pm 0.002$ &  $0.110 \pm 0.007$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.527 \pm 0.002$ &  $0.964 \pm 0.005$ &  $0.047 \pm 0.004$ \\
            &       &         & 5.0 &  $0.752 \pm 0.005$ &  $0.943 \pm 0.002$ &  $0.110 \pm 0.007$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.476 \pm 0.001$ &  $0.949 \pm 0.005$ &  $0.047 \pm 0.005$ \\
            &       &         & 5.0 &  $0.753 \pm 0.006$ &  $0.946 \pm 0.002$ &  $0.103 \pm 0.001$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.468 \pm 0.005$ &  $0.947 \pm 0.002$ &  $0.052 \pm 0.003$ \\
            &       &         & 5.0 &  $0.753 \pm 0.006$ &  $0.946 \pm 0.002$ &  $0.103 \pm 0.001$ \\
\midrule
\multirow{8}{*}{OC} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.500 \pm 0.000$ &  $1.000 \pm 0.000$ &  $0.000 \pm 0.000$ \\
            &       &         & 5.0 &  $0.771 \pm 0.002$ &  $0.943 \pm 0.003$ &  $0.127 \pm 0.004$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.500 \pm 0.000$ &  $1.000 \pm 0.000$ &  $0.000 \pm 0.000$ \\
            &       &         & 5.0 &  $0.771 \pm 0.002$ &  $0.943 \pm 0.003$ &  $0.127 \pm 0.004$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.500 \pm 0.000$ &  $1.000 \pm 0.000$ &  $0.000 \pm 0.000$ \\
            &       &         & 5.0 &  $0.770 \pm 0.001$ &  $0.942 \pm 0.002$ &  $0.126 \pm 0.004$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.500 \pm 0.000$ &  $1.000 \pm 0.000$ &  $0.000 \pm 0.000$ \\
            &       &         & 5.0 &  $0.770 \pm 0.001$ &  $0.942 \pm 0.002$ &  $0.126 \pm 0.004$ \\
\midrule
\multirow{8}{*}{RND} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.447 \pm 0.011$ &  $0.957 \pm 0.001$ &  $0.012 \pm 0.003$ \\
            &       &         & 5.0 &  $0.769 \pm 0.006$ &  $0.943 \pm 0.002$ &  $0.119 \pm 0.006$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.447 \pm 0.011$ &  $0.957 \pm 0.001$ &  $0.012 \pm 0.003$ \\
            &       &         & 5.0 &  $0.769 \pm 0.006$ &  $0.943 \pm 0.002$ &  $0.119 \pm 0.006$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.448 \pm 0.038$ &  $0.957 \pm 0.002$ &  $0.029 \pm 0.030$ \\
            &       &         & 5.0 &  $0.769 \pm 0.003$ &  $0.942 \pm 0.001$ &  $0.126 \pm 0.001$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.448 \pm 0.038$ &  $0.957 \pm 0.002$ &  $0.029 \pm 0.030$ \\
            &       &         & 5.0 &  $0.769 \pm 0.003$ &  $0.942 \pm 0.001$ &  $0.126 \pm 0.001$ \\
\midrule
\multirow{8}{*}{SoftLabeler} & \multirow{4}{*}{False} & \multirow{2}{*}{initial} & 1.0 &  $0.768 \pm 0.009$ &  $0.940 \pm 0.001$ &  $0.224 \pm 0.011$ \\
            &       &         & 5.0 &  $0.733 \pm 0.009$ &  $0.948 \pm 0.002$ &  $0.098 \pm 0.007$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.727 \pm 0.010$ &  $0.941 \pm 0.001$ &  $0.222 \pm 0.011$ \\
            &       &         & 5.0 &  $0.733 \pm 0.009$ &  $0.948 \pm 0.002$ &  $0.098 \pm 0.007$ \\
            & \multirow{4}{*}{True} & \multirow{2}{*}{initial} & 1.0 &  $0.771 \pm 0.005$ &  $0.940 \pm 0.001$ &  $0.222 \pm 0.006$ \\
            &       &         & 5.0 &  $0.735 \pm 0.013$ &  $0.945 \pm 0.002$ &  $0.105 \pm 0.017$ \\
            &       & \multirow{2}{*}{learned} & 1.0 &  $0.725 \pm 0.011$ &  $0.940 \pm 0.001$ &  $0.222 \pm 0.005$ \\
            &       &         & 5.0 &  $0.735 \pm 0.013$ &  $0.945 \pm 0.002$ &  $0.105 \pm 0.017$ \\
\bottomrule
\end{tabular}
}\end{center}
\caption{Out-domain results for measure Native}\label{table:out-domain-Native}
\end{table}

